Unlocking Pixels for Reinforcement Learning via Implicit Attention

There has recently been significant interest in training reinforcement learning (RL) agents in vision-based environments. This poses many challenges, such as high dimensionality and the potential for observational overfitting through spurious correlations. A promising approach to solve both of these problems is an attention bottleneck, which provides a simple and effective framework for learning high performing policies, even in the presence of distractions. However, due to poor scalability of attention architectures, these methods cannot be applied beyond low resolution visual inputs, using large patches (thus small attention matrices). In this paper we make use of new efficient attention algorithms, recently shown to be highly effective for Transformers, and demonstrate that these techniques can be successfully adopted for the RL setting. This allows our attention-based controllers to scale to larger visual inputs, and facilitate the use of smaller patches, even individual pixels, improving generalization. We show this on a range of tasks from the Distracting Control Suite to vision-based quadruped robots locomotion. We provide rigorous theoretical analysis of the proposed algorithm.

==> background.tex <==



Notation taken from \cite{cordonnier2020multihead}. Feel free to change.

\subsection{Attention}

Let $\mathbf{X}~\in~\mathbb{R}^{T\times D_{\textit{in}}}$ and $\mathbf{Y}~\in~\mathbb{R}^{T'\times D_{\textit{in}}}$ be two input matrices consisting of respectively $T$ and $T'$ tokens of ${D_{\textit{in}}}$ dimensions each.
An attention layer maps each of the $T$ query token from $D_{\textit{in}}$ to $D_{\textit{out}}$ dimensions as follows:
\begin{align}
  \hspace{-2mm}\operatorname{Attention}(\textbf{Q}, \textbf{K}, \textbf{V})
  =
  \softmax
  \left(
    \frac{\textbf{Q} \textbf{K}^\top}{\sqrt{d_k}}
  \right)
  \mV, \\
  \label{eq:attention}
\end{align}
$\text{with}\ \mathbf{Q} = \mathbf{X} \mathbf{W}_Q, \mathbf{K} = \mathbf{Y} \mathbf{W}_K,\, \mathbf{V} = \mathbf{Y} \mathbf{W}_V$. The layer is parametrized by a query matrix $\mathbf{W}_Q~\in~\mathbb{R}^{D_{\textit{in}} \times D_{k}}$, a key matrix $\mathbf{W}_K~\in~\mathbb{R}^{D_{\textit{in}} \times D_{k}}$ and a value matrix $\mathbf{W}_V~\in~\mathbb{R}^{D_{\textit{in}} \times D_{\textit{out}}}$.
Using attention on the same sequence (i.e.~$\mathbf{X}=\mathbf{Y}$) is known as self-attention and is the basic building block of the transformer architecture \cite{transformer}. 

\subsection{Multi-Head Attention}

In many cases, multiple attention ``heads'' are concatenated to obtain multi-head attention defined for $N_h$ heads as:
\begin{align}
  \operatorname{MultiHead}(\mathbf{X}, \mathbf{Y}) = \text{concat}_{i \in {[N_h]}}\big[\mathbf{H}^{(i)}\big] \; \mathbf{W}^O \\
  \mathbf{H}^{(i)} = \operatorname{Attention}(\mathbf{X}\mathbf{W}_Q^{(i)}, \mathbf{Y}\mathbf{W}_K^{(i)}, \mathbf{Y}\mathbf{W}_V^{(i)}),
  \label{eq:multi-head-concat}
\end{align}
where distinct parameter matrices $\mathbf{W}_Q^{(i)}, \mathbf{W}_K^{(i)} \in \mathbb{R}^{D_{\textit{in}}\times d_k}$ and $\mathbf{W}_V^{(i)} \in \mathbb{R}^{D_{\textit{in}}\times d_{\textit{out}}}$ are learned for each head $i \in [N_h]$ and the extra parameter matrix $\mathbf{W}^{O}~\in~\mathbb{R}^{N_h d_{\textit{out}} \times D_{\textit{out}}}$ projects the concatenation of the $N_h$ head outputs (each in $\mathbb{R}^{d_{\textit{out}}}$) to the output space $\mathbb{R}^{D_{\textit{out}}}$.
In the multi-head setting, we call $d_k$ the dimension of each head and $D_k=N_hd_k$ the total dimension of the query/key space. For simplicity, we define all parameters for a single attention had as $\mathbf{W}^{(i)} = [\mathbf{W}_Q^{(i)}, \mathbf{W}_K^{(i)}, \mathbf{W}_V^{(i)}]$.


\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{Figures/Method/ModalNet-20.png}
    \vspace{-15mm}
    \caption{A visual representation of multi-head attention from \cite{transformer}.}
    \label{fig:my_label}
\end{figure}


\subsection{Diverse Attention}

In order to measure the diversity of the attention heads, we propose to compute the similarity between two heads using a kernel. Now we can measure the diversity of \textit{all} attention heads as follows:

\begin{definition}\label{Def:div} \textbf{(Attention Diversity)} Consider a finite set of $M$ attention heads, parameterized by $\mathcal{W} = \{\mathbf{W}^{1},...,\mathbf{W}^{M}\}$. We denote
$\mathrm{Div}(\mathcal{W}) \overset{\mathrm{def}}{=} \mathrm{det}( K(\mathbf{H}^{(i)}, \mathbf{H}^{(j)})_{i,j=1}^M) = \mathrm{det}(\mathbf{K})$,
% \label{equation:pop_div}
where $K:\mathbb{R}^{l} \times \mathbb{R}^{l} \rightarrow \mathbb{R}$ is a given kernel function. Matrix $\mathbf{K}$ is positive semidefinite since all principal minors of $\mathrm{det}(\mathbf{K})$ are nonnegative.
\end{definition}

\jcom{need different notation for the kernel matrix since the key matrix is $\mathbf{K}$}

This formulation is heavily inspired by Determinantal Point Processes (DPPs, \cite{Kulesza}), a mechanism which produces diverse subsets by sampling proportionally to the determinant of the kernel matrix of points within the subset. From a geometric perspective, the determinant of the kernel matrix represents the volume of a parallelepiped spanned by feature maps corresponding to the kernel choice. We seek to maximize this volume, effectively ``filling'' the feature space. 

Now consider the joint loss function, as follows:
\begin{equation}
\label{eqn:div_transformer}
    J(\mathcal{W}) = \underbrace{\mathcal{L}(\mathcal{W})}_\text{loss function} \; + 
    \underbrace{%
     \lambda \mathrm{Div}(\mathcal{W})}_{\text{head diversity}}
\end{equation}

where $\lambda_t \in (0,1)$ is the trade-off between reward and diversity. Note that the diversity will be equal to zero if any two rows of the kernel matrix are linearly dependent, which means this loss function naturally focuses on making no two heads the same, rather than maximizing pairwise difference. 

In addition, note that $\mathrm{log} (\mathrm{det} (\mathbf{K}))$ is differentiable. 


\begin{table}[h]
    \centering
    \caption{\small{WikiText2, four encoder layers, embedding dim=200, hiddensize=200, ten epochs. Three seeds, mean $\pm$ standard deviation.}}
    \scalebox{1.0}{
    \begin{tabular}{l*{3}{c}r}
    \toprule
    \textbf{Beta} & $\mathbf{M=4}$ & $\mathbf{M=8}$ \\
    \midrule
    0 & 103.51 $\pm$ 1.6 & 99.63 $\pm$ 1.31 \\
    0.0001 & 101.98 $\pm$ 2.35 & 99.32 $\pm$ 0.73\\
    0.001 & \textbf{101.09} $\pm$ 1.23 & \textbf{99.23} $\pm$ 1.54\\
    0.01 &  419.90 $\pm$ 264.7 & 368.11 $\pm$ 96.93\\
    \bottomrule
\end{tabular}}
\end{table}
\label{table:initial_wikitext2}

\begin{table}[h]
    \centering
    \caption{\small{WikiText2, five encoder layers, embedding dim=200, hiddensize=1000, ten epochs. Three seeds, mean $\pm$ standard deviation. Adam, lr=0.0003, bptt=200.}}
    \scalebox{1.0}{
    \begin{tabular}{l*{3}{c}r}
    \toprule
    \textbf{Beta} & $\mathbf{M=5}$ & $\mathbf{M=10}$ \\
    \midrule
    0 & 80.01 $\pm$ 0.26 & -  \\
    0.001 & 79.58 $\pm$ 0.56 & - \\
    0.01 & 79.85 $\pm$ 0.92 & - \\
    0.1 &  \textbf{79.27}  $\pm$ 0.26 &  - \\
    1 &  79.73  $\pm$ 0.88 &  - \\
    \bottomrule
\end{tabular}}
\end{table}
\label{table:initial_wikitext2}


\subsection{Learning Diverse Kernels}

The other approach would be to learn different kernels for different heads. Instead of preprocessing $\mathbf{X}$ with $\mathbf{W}_{Q}$, $\mathbf{W}_{K}$ and $\mathbf{W}_{V}$, one can obtain query/key/value matrices by passing $\mathbf{X}$ through neural network with positive nonlinear mappings $f:\mathbb{R} \rightarrow \mathbb{R}_{+}$: $\mathcal{N}_{Q}$, $\mathcal{N}_{K}$, $\mathcal{N}_{V}$. The attention matrix would be then given as:
\begin{equation}
\label{decomposition}
\mathbf{A} = \mathcal{N}_{Q}(\mathbf{X}) \mathcal{N}_{K}(\mathbf{X})^{\top}.   
\end{equation}

Diversity across different heads can be done quantified by the diversity between corresponding learned kernels.

That brings us to the question, how to measure similarity/dissimilarity between different similarity measures.

Before answering that question, lets us emphasize that Eq. \ref{decomposition} proposed attention matrix $\mathbf{A}$ that can be decomposed and thus does not need to stored explicitly in the memory to compute the results of the attention block. Note that the not-normalized attention produces matrix of the form $\mathbf{AV}$ that, according to Eq. \ref{decomposition} can be rewritten as:
\begin{equation}
\mathbf{AV} = \mathcal{N}_{Q}(\mathbf{X}) (\mathcal{N}_{K}(\mathbf{X})^{\top}\mathbf{V}),
\end{equation}
where brackets on the RHS indicate order of computations.
Notice that RHS can be computed in time $O(Lmd)$, where $L$ is the length of the input sequence, $d$ is the dimensionality of the embeddings $\mathbf{x}_{i}$ and $m$ is the size of the final layers of neural networks $\mathcal{N}_{Q}$ and $\mathcal{N}_{K}$.

Completely analogous analysis can be conducted for the normalized attention block.

\section{Diverse Attention via Kernel Distances}

Consider again the sequence of embeddings of the input tokens encoded as a matrix $\mathbf{X} \in \mathbb{R}^{L \times d}$.
For each fixed token $i$ and its embedding $\mathbf{x}_{i}$, we take the corresponding $i^{th}$ row $\mathbf{a}_{i}$ of the attention matrix $\mathbf{A} \in \mathbb{R}^{L \times L}$. This row encodes a discrete (softmax if regular attention model is used) distribution over the set of all the embeddings $\{\mathbf{x}_{1},...,\mathbf{x}_{L}\} \subseteq \mathbb{R}^{d}$. We call it $\mathcal{P}^{h}_{i}$, where $h$ is an index identifying particular head being used.

Given fixed $i$ and two heads indexed by $h_{1}$ and $h_{2}$ and a fixed kernel $K:\mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$ (that will be acting on embeddings $\mathbf{x}_{i}$), we can now compute the \textit{cross-similarity} between 
distributions $\mathcal{P}^{h_{1}}_{i}$ and
$\mathcal{P}^{h_{2}}_{i}$ as follows:
\begin{equation}
\mathcal{K}(\mathcal{P}^{h_{1}}_{i}, \mathcal{P}^{h_{2}}_{i}) =  
\sum_{a \in \{1,...,L\}}\sum_{b \in \{1,...,L\}}
p^{h_{1}, i}_{a}p^{h_{2}, i}_{b}K(\mathbf{x}_{a},\mathbf{x}_{b}),
\end{equation}
where $p^{h, i}_{c}$ is a probability corresponding to $c^{th}$ embedding $\mathbf{x}_{c}$ in discrete distribution $\mathcal{P}^{h}_{i}$.

Such kernels computed between probabilistic distributions can be then used to compute similarity kernel between two heads indexed by $h_{1}$ and $h_{2}$ for instance as follows (this is just one of many possibilities):
\begin{equation}
\widehat{K}(h_{1}, h_{2}) = \frac{1}{L} \sum_{i=1}^{L} \mathcal{K}(\mathcal{P}^{h_{1}}_{i}, \mathcal{P}^{h_{2}}_{i}).     
\end{equation}

\textbf{Such a kernel can be piped-in to the determinant-trick.}

Note also that for a similarity measure $\mathcal{K}$, there is a natural notion of the accompanying distance $D^{h_{1},h_{1}}_{i}$ with its square defined as follows:
\begin{equation}
(D^{h_{1},h_{1}}_{i})^{2} = \mathcal{K}(\mathcal{P}^{h_{1}}_{i}, \mathcal{P}^{h_{1}}_{i}) + \mathcal{K}(\mathcal{P}^{h_{2}}_{i}, \mathcal{P}^{h_{2}}_{i}) - 2\mathcal{K}(\mathcal{P}^{h_{1}}_{i}, \mathcal{P}^{h_{2}}_{i}).
\end{equation}





==> preliminaries.tex <==

\section{Self-Attention Bottlenecks in RL}

Intro to Yujins approach, ES formulation, etc. Possible diagram.

==> workspace.tex <==
To summarize, our key contributions are as follows: 
\begin{itemize}
    \item \textbf{Practical}: To the best of our knowledge, we are the first to use efficient attention mechanisms for RL from pixels. This has two clear benefits: \textbf{1)} we can scale to larger images than previous works; \textbf{2)} we can use more fine-grained patches which produce more effective attention bottlenecks. Both goals can be achieved with an embarrassingly small number of trainable parameters for vision processing (\textbf{8x} compression over standard CNN-based policies with no loss of quality of the learned controller). Furthermore, IAP-rank provides \textbf{interpretability} since those regions of the image that an agent pays attention to can be easily visualized and IAP-trans achieves image \textbf{compression}. Both are CNN-free. We test IAP on a rich set of tasks including: Distracting Control Suite \cite{distracting}, navigation, obstacle avoidance and quadruped robot walking in uneven terrain. 
    
    \item \textbf{Theoretical}: We provide rigorous theoretical analysis of IAP, showing in particular that linearization of the attention combined with ranking can leverage a rich class of algorithms on dot-product maximization and nearest neighbor search and quantifying the quality of those IAP variants that apply approximate softmax kernel estimation techniques. 
\end{itemize}
